To What Extent do Open-loop and Feedback Nash Equilibria Diverge in General-Sum Linear Quadratic Dynamic Games?

Dynamic games offer a versatile framework for modeling the evolving interactions of strategic agents, whose steady-state behavior can be captured by the Nash equilibria of the games. Nash equilibria are often computed in feedback, with policies depending on the state at each time, or in open-loop, with policies depending only on the initial state. Empirically, open-loop Nash equilibria (OLNE) could be more efficient to compute, while feedback Nash equilibria (FBNE) often encode more complex interactions. However, it remains unclear exactly which dynamic games yield FBNE and OLNE that differ significantly and which do not. To address this problem, we present a principled comparison study of OLNE and FBNE in linear quadratic (LQ) dynamic games. Specifically, we prove that the OLNE strategies of an LQ dynamic game can be synthesized by solving the coupled Riccati equations of an auxiliary LQ game with perturbed costs. The construction of the auxiliary game allows us to establish conditions under which OLNE and FBNE coincide and derive an upper bound on the deviation between FBNE and OLNE of an LQ game.

==> Draft_introduction.tex <==

Autonomous systems are increasingly deployed across a wide range of multi-agent interactive settings. Examples range from self-driving vehicles operating in urban traffic to assistive robotics for the disabled. However, autonomous systems today often struggle to infer the intent of humans or other autonomous systems in their environment, and to accurately predict the impact of their actions on others' decision-making. The inability of autonomous agents to accurately infer others' objectives and anticipate others' reactions frequently results in unsafe and inefficient interactions, such as autonomous-vehicle related collisions.

To address these shortcomings, dynamic game theory has recently emerged as a powerful mathematical framework for modeling interdependent reasoning in multi-agent interactions. In recent years, the dynamic game theory community has developed efficient algorithms for computing the \textit{Nash equilibria} of a \textit{forward} dynamic game, which encode steady-state modes of interaction at which each agent's strategy is unilaterally optimal with respect to their cost objective. Other works have focused on solving \textit{inverse} dynamic games, the problem of inferring the unknown cost objectives of interacting dynamic agents from noisy trajectory data. In both forward and inverse games, ...

~\\
\frank{Something about how \textit{information pattern} plays a pivotal role in  both forward and inverse games.}
~\\

